AI Governance through Markets

This paper argues that market governance mechanisms should be considered a key approach in the governance of artificial intelligence (AI), alongside traditional regulatory frameworks. While current governance approaches have predominantly focused on regulation, we contend that market-based mechanisms offer effective incentives for responsible AI development. We examine four emerging vectors of market governance: insurance, auditing, procurement, and due diligence, demonstrating how these mechanisms can affirm the relationship between AI risk and financial risk while addressing capital allocation inefficiencies. While we do not claim that market forces alone can adequately protect societal interests, we maintain that standardised AI disclosures and market mechanisms can create powerful incentives for safe and responsible AI development. This paper urges regulators, economists, and machine learning researchers to investigate and implement market-based approaches to AI governance.

==> Disclosure_Old.tex <==
\section{Disclosing AI’s development and deployment}

\subsection{Disclosure: A Primer}

Disclosure refers to the process of releasing all relevant information pertaining to a company. It is the foundation of the aforementioned market governance mechanisms as disclosure powers auditing, insurance, due-diligence and procurement. Disclosure can be financial or non-financial \cite{vanstraelen2003disclosure, musweu2018disclosure}.

Central to financial disclosures are financial statements—comprising the balance sheet, income statement, and cash flow statement—which collectively provide insights into a firm’s financial position, operational performance, and liquidity \cite{hassan2019measurement}. The global standardisation of these practices is governed by the International Financial Reporting Standards (IFRS) \cite{vangreuning2011ifrs} and, in the United States, by Generally Accepted Accounting Principles (GAAP)\cite{wustemann2021gaap}. These regulatory frameworks impose detailed requirements concerning the content, format, and timing of financial disclosures to ensure stakeholders receive timely, relevant, and accurate information. The enforcement of these standards is overseen by bodies such as the Securities and Exchange Commission (SEC) in the United States, with non-compliance subject to legal penalties \cite{sec1945}. 

Non-financial reporting encompasses the disclosure of a company's operations, business risks, and corporate strategies that are not captured in traditional financial statements \cite{turzo2022nonfinancial}. Efficient markets rely on minimising information asymmetry through transparent disclosures to ensure that all relevant information is reflected in asset prices \cite{perrini2006practitioner}. High-quality non-financial disclosures can reduce the cost of capital, thereby levelling the playing field for all investors and contributing to a more efficient capital market \cite{cuadrado2016corporate}.

Most non-financial disclosures are not obligatory in the majority of jurisdictions. Nevertheless, 1,395 investors, who collectively manage \$59 trillion—accounting for 60\% of global assets under management—have endorsed the UN Principles of Responsible Investment (UN PRI) \cite{pri2024annual}. This endorsement signifies a commitment to, among other considerations, take non-financial disclosures into account when making investment decisions. Instances of widespread, non-financial disclosures encompass research and development (R\&D) information \cite{koh2014rd}, sustainability reports \cite{saini2022disclosures}, and organisational practices \cite{arvidsson2011disclosure}.

Some funds will include or exclude potential investments on the basis of their non-financial information \cite{curtis2021esg, dikolli2022esg}. Vanguard's Environmental, Social, and Governance (ESG) fund focuses on investing in companies with strong environmental practices, excluding those with significant involvement in fossil fuels or other industries that have a negative environmental impact, while promoting sustainability and responsible corporate governance \cite{hill2020esg}. R\&D disclosure is positively associated with investor attention towards firms, yet it may also expose commercially sensitive information to competitors \cite{baruffaldi2024asymmetric}. Thus, a delicate balance must be struck between materiality and sensitivity, especially since said disclosure is discretionary in almost all cases. This discretion leads to significant discrepancies in the quality and description of non-financial disclosures \cite{gao2016disclosure}.

Crucial for our purposes, non-financial disclosures provide market actors with information on potential risks that may not be immediately apparent from financial statements \cite{pozzoli2022nonfinancial, flostrand2006valuation}. We observe for instance, that governance structures can reveal risks such as regulatory fines or the potential for corporate scandals \cite{borodin2019statements}.

Non-financial disclosures also reflect investor demand \cite{thewissen2024esg}. There is large investor demand for non-financial. There are over 3,551 unique SASB reporters and 2,600 organisations supporting TCFD recommendations as of 2022 \cite{ifrs_sasb}. For example, it is common for investors to prefer funds that do not invest in companies providing services to the military \cite{starr2008sri}. Moreover, regulatory compliance and incentives related to non-financial factors can significantly impact asset pricing. Companies excelling in environmental, social, and governance reporting may benefit from regulatory incentives or avoid penalties, thereby affecting their financial health and market valuation \cite{mbir2020ifrscg}.

\subsection{AI Disclosures}

Standardisation serves to simplify complex risk areas, rendering them accessible to a broad range of market participants who may lack expertise in AI.  By adopting a common framework, AI risks can be articulated in a manner that facilitates more informed decision-making across investment, insurance, and procurement activities. The absence of a standardised approach to reporting AI-related risks introduces significant challenges for investors, insurers, and other stakeholders. Without uniform metrics, assessing the financial and operational implications of AI risks becomes difficult, resulting in inefficiencies in capital allocation and decision-making processes. A standardised risk framework is essential, as it provides consistent and comprehensible metrics for communicating complex AI risks to non-specialists within the market. While such frameworks may not fully capture the intricacies of each risk, they serve as a practical means of ensuring that AI-related concerns can be communicated and addressed effectively.

We argue that the AI research communities can contribute to AI governance by standardising the disclosure of AI. This standardisation requires the consistent description and quantification of key aspects of AI systems - to enable firms, policymakers and other actors to make informed decisions. 

Providers, such as developers of foundational general-purpose AI systems like GPT-4o, create the underlying models, while distributors use these models to offer products, such as ChatGPT \cite{gutierrez2023gpa}. A growing community of researchers in academia, civil society, government, and industry are actively studying the risks associated with AI. These risks are not always negative, but rather descriptions of various features of the AI models and organisations that develop or distribute them that are currently uncertain. These risks are increasingly communicated through various market governance mechanisms. For instance, organisations like METR, which function as safety auditors, evaluate the risk profiles of companies like Anthropic or OpenAI \cite{achiam2023gpt4}. Over this decade, the standardisation of how AI-related information is transmitted through markets will likely solidify, much as we already see with performance benchmarks such as GPQA \cite{rein2023gpqa}, MATH \cite{hendrycks2021math}, and MMLU \cite{hendrycks2020massive} being widely adopted by companies like OpenAI, DeepMind, and Anthropic.

In a competitive environment, the pressure to reduce risk becomes even more pronounced. AI companies that successfully minimise risk can gain a competitive edge by attracting capital, securing better terms, and winning more procurement contracts. This competitive advantage can create a virtuous cycle where reducing risk not only enhances a company’s market position but also encourages industry-wide adoption of safer practices. As competitors observe the benefits of risk reduction, they too will be motivated to improve their risk profiles, leading to a broader industry shift towards safer AI development and deployment.

By establishing clear guidelines for describing risks— such as the allocation of compute, incident reporting, and capabilities in various areas—organisations can provide a comprehensive view of their AI models' vulnerabilities and limitations. This would be paired with specific metrics to quantify these risks, such as model error rates, data privacy breach incidents, or energy consumption during model training and deployment. Such quantification enables stakeholders to make more informed comparisons between different AI systems and providers. With standardised reporting, market actors can assess AI risks more accurately, reducing uncertainty and promoting better capital allocation. 

The aforementioned market governance mechanisms all require a framework of AI disclosure that identifies different sources of risk. To disclose requires an understanding of the different areas that are present in the development and deployment of AI, as well as in the organisations that develop and deploy. For example, OpenAI's preparedness framework identifies categories such as: 1) Individualised persuasion, 2) Cybersecurity, 3) Chemical, biological, radiological, and nuclear threats, and Autonomous replication and adaptation \cite{openai2023preparedness}. Many other such frameworks exist, with the AI Risk Repository capturing 700+ risks extracted from 43 existing frameworks \cite{slattery2024risks}. As such, this present paper will not be providing an exhaustive literature review of different AI Risks. 

For the purpose of standardizing AI Risk disclosure, two critical aspects must be emphasized. First, Risk should not be construed as inherently negative but rather as associated with uncertainty. A risk area is an area of uncertainty. Second, the way in which different aspects of AI are disclosed needs to be standardised in order for them to be utilised by and communicated between different market actors. This involves turning a complex nuanced area into a single metric or groups of metrics \cite{tate2007standardisation}. Some standardised metrics have already emerged, such as the size of models expressed with floating-point operations per second (FLOPS) \cite{chen2023flops}, and the generalised capability of AI being regularly disclosed with famous benchmarks such as GPQA, MMLU and MATH \cite{rein2023gpqa, hendrycks2020massive,  hendrycks2021math}. More metrics will be needed in order to fully describe the vast range of potential applications of AI. 

\subsection{The Large Model Production Line}

Standardised metrics of AI risk will describe different aspects of AI development and deployment. The development of large models—encompassing large language models, reasoning models, multimodal models, and other advanced AI systems—follows a production pipeline with clearly delineated stages, each of which plays a critical role in shaping the model's capabilities \cite{dubey2024llama}. The process initiates with data acquisition, where diverse datasets are curated and selected. This stage involves extensive data curation, filtering out low-quality or biased data, and ensuring compliance with privacy regulations like GDPR through anonymisation \cite{liu2024understanding}. These datasets are subsequently subjected to tokenisation and preprocessing, which includes normalising text, balancing data, and preparing it for model consumption.

Pre-training follows, where models are exposed to extensive datasets, learning foundational patterns \cite{du2024stacking}. This stage is informed by scaling laws that balance data volume, model size, and compute resources to optimise performance. It is succeeded by mid-training, a phase that includes fine-tuning for specific tasks, domain adaptation, and multi-task learning \cite{parthasarathy2024ultimate}. Here, models are specialised to handle targeted applications and may be refined based on emergent insights or additional data.

Before proceeding to post-training, models undergo rigorous evaluation using benchmarks to test their accuracy, robustness, fairness, and other \cite{hodak2023benchmarking}. This ensures models meet technical and saftey standards before further refinement. Evaluation and benchmarking also takes place at earlier later stages. Post-training includes reinforcement learning from human feedback (RLHF) and other techniques, as well as additional safety work such as audits, red-teaming, and capability enhancement like teaching tool use \cite{ouyang2022training, wei2024jailbroken, mazeika2024harmbench}. These steps ensure the model aligns with user needs and regulatory expectations.

Upon completing these stages, models are prepared for productisation, where they are optimised for deployment environments, such as through quantisation or distillation to reduce computational load  \cite{wang2024art, sreenivas2024llm}. This stage ensures that models are both efficient and effective for commercial applications. Deployment involves integrating models into production systems, accompanied by continuous monitoring to track performance and detect issues like data drift \cite{jang2024driftwatch}. Finally, post-deployment feedback loops allow for ongoing model improvement, incorporating new data to keep models aligned with evolving user needs and market demands \cite{shi2024continual}.

Within this production pipeline, a number of aspects are of material significance to market participants, including investors, regulators, and insurers. A detailed understanding of the risks, methodologies, and safeguards associated with each stage is essential for accurately assessing the potential returns and liabilities inherent in the development of large models. Enhanced transparency throughout these processes can facilitate improved risk assessment, inform capital allocation decisions, and ensure compliance with regulatory frameworks, thereby supporting models that meet stringent safety, ethical, and performance benchmarks.

This section outlines some standardisation targets that are anticipated to become prevalent across various stages of the large model production process. Companies are already disclosing some of these metrics. These projections are grounded in current regulatory requirements, industry best practices, and emergent trends in AI governance. It is important to note that this is not an exhaustive inventory. Future research should extend this, providing a more comprehensive perspective on the requisite standards for developing responsible and market-aligned models.

\begin{figure}[ht]
    \centering
    \makebox[\textwidth][c]{%
        \includegraphics[width=1.4\textwidth]{diagram2.png} % Makes the figure 120% of text width
    }
    \caption{The 8 macro stages of the large AI model production line. This is a simplified overview. Other stages are described in the article text. This is not a comprehensive overview of large AI model development.}
    \label{fig:diagram2}
\end{figure}



\subsubsection{Data Acquisition and Privacy in AI Systems}

Data acquisition is a foundational step in developing large models, as the quality and diversity of datasets directly influence the performance and reliability of AI systems. This stage requires careful attention to privacy regulation especially given the legal landscapes (e.g., GDPR). As such, standardised reporting in this domain might include metrics related to data provenance, detailing the sources and methods of data collection—whether through scraping, crowd sourcing, or third-party purchases — and providing transparency on labelling practices. Recent legal challenges, such as lawsuits against AI companies for using copyrighted materials \cite{reuters2024anthropic, copyright2023courts} underscore the importance of curating datasets to exclude unauthorised content. A core issue in data privacy relates to how personal information is managed and protected during and after collection. High-performance models often require substantial data retention, which can inadvertently include sensitive information \cite{el2022impossible}. Private data, such as contact numbers and email addresses, can remain within training datasets and be extracted from models \cite{carlini2022quantifying}.

Companies can provide standardised disclosures on their data practices. This could include descriptions of data minimisation efforts, encryption standards, data anonymisation techniques, data storage practices, retention periods, and the purposes for which data is used. Disclosures may also cover details on third-party access to data, as well as how companies handle data subject requests, such as access, rectification, or erasure of personal information. Transparent reporting on data breaches—such as the number of sensitive records exposed, their nature, and mitigation measures—could further aid market participants in assessing a company’s risk management capabilities. Where appropriate, companies can employ existing standardisation metrics from frameworks such as the ISO/IEC 27001 for information security \cite{ganji2019approaches}, and the NIST Privacy Framework \cite{hiller2017privacy}.


\subsubsection{Energy: Data Centre Efficiency and Algorithm Design}

Large AI models have large energy demands, driving the need for energy-efficient infrastructure and algorithms. Data centre efficiency methods aim to optimise the energy use of computational resources to support model training. This includes strategies for aligning workload demands, resource allocation, and energy balancing \cite{chong2013data}, alongside software-oriented approaches for workload management \cite{khan2022workload}, and integrated power management strategies \cite{mittal2014power}. Simultaneously, algorithm design plays a critical role in improving the energy efficiency of machine learning processes, with techniques like federated edge learning \cite{mo2021energy}, hardware acceleration \cite{zeng2023energy}, and sparsely activated deep neural networks \cite{patterson2021carbon} offering significant reductions in energy consumption.

Standardised reporting on data centre efficiency might include energy consumption metrics like Power Usage Effectiveness (PUE) and the proportion of energy derived from renewable sources \cite{jaureguialzo2011pue}. Companies could also disclose which energy sources they use. For algorithm design, companies could report on energy efficiency metrics related to training processes, detailing how different techniques reduce the computational burden. Frameworks like the GRI \cite{petera2015global}, ISO 50001 \cite{marimon2017reasons}, and The Green Grid \cite{jaureguialzo2011pue} can already provide some reporting guidelines. 

\subsubsection{Compute Allocation}

Describing the allocation of compute resources would reveal information about the production processes and the safety measures applied throughout AI model development. Market actors could understand a company's strategic focus. For example, companies could disclose the quarterly compute spend on pre-training, mid-training, post-training, safety work, and inference \cite{dubey2024llama, liu2024understanding}. This macro overview could market participants, such as investors performing due diligence, evaluate where a company places its resources and how it balances the goals of innovation, safety, and efficiency.

\subsubsection{Intended Model Behaviour}

Large model developers use a series of different method to shape their model's behaviour. This involves shaping model outputs to prioritise valuable behaviours while preventing unsafe, illegal, or unethical content. Techniques such as RLHF \cite{ouyang2022training}, Direct Preference Optimisation (DPO) \cite{rafailov2024direct}, fine-tuning \cite{parthasarathy2024ultimate}, red-teaming \cite{mazeika2024harmbench}, and output filters \cite{li2023unlocking} are commonly employed to align model outputs with desired outcomes to ensure models remain safe for public use. A great focus is placed on avoiding unwanted behaviours, which result in reputational risks and legal liabilities. Key areas of concern include avoiding, harmful content, such as suicide ideation \cite{bhaumik2023mindwatch}, "hallucinations" \cite{Kaddour2023ChallengesAA}, and bias in model outputs \cite{Oketunji2023LargeLM}.

To standardise disclosures related to intended model behaviour, companies could report on their intended model behaviours, and the methods and processes that they are employing to achieve these intended behaviours. The OpenAI Model Spec provides a strong example of transparency in this area \cite{openai2024model_spec}. It details how it wants its models to behave, whilst trying to align with specific ethical objectives, safety measures, and user needs, balancing user directives with broader considerations like legality and societal impact. 

\subsubsection{Model Interpretability}

Model interpretability involves methods that enhance the transparency and understanding of AI systems \cite{Gunning2019DARPAsEA}. Often, AI models function as "black boxes," making it difficult to understand the reasoning behind their predictions. \textit{Explainable AI} \cite{Linardatos2020ExplainableAA} and \textit{Mechanistic Interpretability} \cite{Conmy2023TowardsAC} offer techniques for clarifying the logic behind model outputs, helping stakeholders gain better insights into the model's decision-making process.

Companies could standardise the disclosure of interpretability techniques to provide insights into how specific decisions are made. They might also disclose aspects of model architecture, any identified biases or limitations. There are technical breakthroughs that need to be made for this to be fully possible, but setting standards also sets a research aim. Frameworks like the Foundation Model Transparency Index  \cite{Bommasani2023TheFM} could guide some of these disclosures.

\subsubsection{Open-source practices}

Open-source practices in AI development allow developers to share code, datasets, and methodologies \cite{Shrestha2023BuildingOA}. This openness can accelerate progress and enable efficient peer review to identify and rectify errors. Open-sourcing advanced AI models can also come with risks, such as model poisoning and dual-use concerns (e.g., repurposing models for harmful  applications) \cite{Eiras2024RisksAO}. Additionally, transparency can challenge intellectual property (IP) management and compliance with data privacy laws.

To standardise open-source practices, companies might disclose detailed documentation of their open-source contributions, including code, datasets, and methodologies. Disclosing incidences of potential dual-use cases can aid regulatory bodies in understanding associated risks. Companies could also outline governance structures for contributions and establish clear policies for IP rights (IPR) and licensing, particularly when integrating open-source elements into commercial products. Companies can use aspects of existing frameworks like the Open Source Initiative \cite{initiative2004opensource} for licensing, or the Linux Foundation’s OpenChain Specification \cite{Coughlan2020StandardizingOS} for open-source compliance.

\subsubsection{Adversarial Testing}

Adversarial testing assesses the resilience of AI systems by exposing them to challenging inputs designed to exploit vulnerabilities. These methods are essential for evaluating how AI models withstand malicious attempts, especially in security-sensitive applications \cite{ruiz2022adversarial}. They help identify risks like data poisoning, evasion attacks, and extraction threats, which can compromise model integrity \cite{hannon2024resiliency}. 

Companies could standardise disclosures by detailing adversarial risks identified during testing. Reporting the scale, frequency, and outcomes of these tests, as well as the data sources, can provide stakeholders with insights into a model's robustness \cite{Croce2020RobustBenchAS}.

\section{Discussion}

\subsection{A Research Agenda: Translating AI Knowledge into Metrics}

\begin{figure}[ht]
    \centering
    \makebox[\textwidth][c]{%
        \includegraphics[width=1.4\textwidth]{diagram3.png}  % Makes the figure 120% of text width
    }
    \caption{The steps towards developing AI risk disclosure metrics.}
    \label{fig:diagram3}
\end{figure}


To fully realise the potential of these market governance mechanisms in mitigating AI risks, the AI safety, ethics, policy, and governance communities must play a proactive role. These communities possess deep expertise in identifying and understanding the nuances of AI-related risks, and their insights are crucial for developing standardised frameworks that can be communicated effectively within the market. By translating their research into standardised information that can be easily understood and utilised by investors, insurers, and procurers, these communities can help bridge the information gap. This standardisation would not only make it easier for markets to assess and manage AI risks but also ensure that the right incentives are in place for AI companies to prioritise safety and ethical considerations in their development process. However, for this expertise to be useful to market participants it must be distilled into metrics that clearly communicate the associated risks and benefits. The challenge for researchers is to reduce complex, technical insights into market signals.

The first step for researchers is to identify the core risks in current AI systems. Again, these risks represent areas of uncertainty, which can produce either positive or negative outcomes. These risks can relate to anything from model capability, to model bias, and cybersecurity. Each of these risks can have real-world implications, such as financial losses or gains, reputational damage, or legal liabilities, making them critical for market actors to assess. Researchers need to frame these risks in ways that align with market concerns, effectively bridging the gap between technical AI knowledge and its economic and regulatory consequences.

Once key risks are identified, the next task is to develop measurable metrics that quantify these risks. Researchers must design metrics that accurately reflect aspects of AI models and the organisations that develop or deploy them. This involves distilling multifaceted technical concepts into single, actionable figures or indices that can be consistently measured across different models and applications. The challenge is to ensure that these metrics maintain their accuracy and relevance while being simple enough for market actors to understand and use.

Furthermore, researchers need to ensure that their metrics are actionable for relevant market participants. Engaging with investors, regulators, and industry representatives can help researchers understand how their metrics are interpreted and whether they guide decision-making effectively. This feedback is crucial for refining the metrics and making sure they serve as practical tools for risk management. The goal is not only to inform stakeholders of potential risks but to drive actions that mitigate those risks, such as adjustments to AI deployments or increased human oversight.

Finally, the AI risk metrics should be validated. A metric should capture the concept it is aiming to capture, whilst doing so consistently, across different models and contexts. Data on metrics should be gathered on a regular basis (e.g., once a quarter) to detect changes stemming from updated model architecture, new data, and use of computing.

In addition, there may be trade-offs between generalised and industry-specific metrics. Each industry will have its unique set of dynamics and risks, as well as regulatory requirements. The risks associated with autonomous vehicles (namely safety and liability) are different from those trading algorithms (market volatility risks).
